DQM: Decentralized Quadratically Approximated Alternating Direction Method of Multipliers

This paper considers decentralized consensus optimization problems where nodes of a network have access to different summands of a global objective function. Nodes cooperate to minimize the global objective by exchanging information with neighbors only. A decentralized version of the alternating directions method of multipliers (DADMM) is a common method for solving this category of problems. DADMM exhibits linear convergence rate to the optimal objective but its implementation requires solving a convex optimization problem at each iteration. This can be computationally costly and may result in large overall convergence times. The decentralized quadratically approximated ADMM algorithm (DQM), which minimizes a quadratic approximation of the objective function that DADMM minimizes at each iteration, is proposed here. The consequent reduction in computational time is shown to have minimal effect on convergence properties. Convergence still proceeds at a linear rate with a guaranteed constant that is asymptotically equivalent to the DADMM linear convergence rate constant. Numerical results demonstrate advantages of DQM relative to DADMM and other alternatives in a logistic regression problem.

==> bibi.tex <==
\begin{thebibliography}{6}

\bibitem{Ribeiro10}
A.~Ribeiro, \emph{Ergodic stochastic optimization algorithms for wireless communication and networking}, .\hskip 1em plus
  0.5em minus 0.4em\relax IEEE Trans. Signal Process., vol. 58, no. 12, pp. 6369-6386, December 2010.
\\    
\bibitem{Ribeiro12}
A.~Ribeiro, \emph{Optimal resource allocation in wireless communication and networking}, .\hskip 1em plus
 0.5em minus 0.4em\relax EURASIP J. Wireless commun., vol. 2012, no. 272, August 2012.
\\    
\bibitem{Broyden}
C.~G.~Broyden,~J.~E.~Dennis~Jr. and ~J.~J.~More, \emph{On the local and superlinear convergence of quasi-Newton methods}, .\hskip 1em plus
 0.5em minus 0.4em\relax IMA J. Appl. Math, vol. 12, Issue 3, pp. 223-245, 1973.    
\\    
\bibitem{Byrd}
R.~H.~Byrd,~J.~Nocedal and~Y.~Yuan, \emph{Global convergence of a class of quasi-Newton methods on convex problems}, .\hskip 1em plus
 0.5em minus 0.4em\relax SIAM J. Numer. Anal., vol. 24, Issue 5, pp. 1171-1190, October 1987.     
 \\
 \bibitem{Nocedal}
J.~Nocedal and S.~J.~Wright, \emph{Numerical optimization}, 2nd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Springer Series in Operations Research. Springer-Verlag, New York, NY., 1999.    
  \\
  \bibitem{Powell}
Powell,~M.~J.~D., \emph{Some properties of the variable metric method}, 2nd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax In numerical methods for non-linear optimization, London: Academic Press, 1972.     
\\
\bibitem{Boyd}
S.~Boyd and L.~Vandenberghe, \emph{Convex Optimization}, \hskip 1em plus
  0.5em minus 0.4em\relax Cambridge, U.K.: Cambridge Univ. Press, 2004.    
\\
\bibitem{Solo}
V.~Solo and X.~Kong, \emph{Adaptive Signal Processing Algorithms: Stability
and Performance} \hskip 1em plus
  0.5em minus 0.4em\relax Englewood Cliffs, NJ: Prentice-Hall, 1995.
  
\end{thebibliography}
